Progressive Transactional Memory in Time and Space

Transactional memory (TM) allows concurrent processes to organize sequences of operations on shared \emph{data items} into atomic transactions. A transaction may commit, in which case it appears to have executed sequentially or it may \emph{abort}, in which case no data item is updated. The TM programming paradigm emerged as an alternative to conventional fine-grained locking techniques, offering ease of programming and compositionality. Though typically themselves implemented using locks, TMs hide the inherent issues of lock-based synchronization behind a nice transactional programming interface. In this paper, we explore inherent time and space complexity of lock-based TMs, with a focus of the most popular class of \emph{progressive} lock-based TMs. We derive that a progressive TM might enforce a read-only transaction to perform a quadratic (in the number of the data items it reads) number of steps and access a linear number of distinct memory locations, closing the question of inherent cost of \emph{read validation} in TMs. We then show that the total number of \emph{remote memory references} (RMRs) that take place in an execution of a progressive TM in which $n$ concurrent processes perform transactions on a single data item might reach $\Omega(n \log n)$, which appears to be the first RMR complexity lower bound for transactional memory.

==> disc.tex <==
%!TEX root = prog.tex
\section{Concluding remarks}
\label{sec:disc}
%
Theorem~\ref{th:iclb} improves on the result in \cite{tm-book} concerning the overhead of validation imposed on
TM implementations that employ invisible reads. We believe that the TM-progress and TM-liveness restrictions
as well as the definitions of DAP and invisible reads we consider for this result are the weakest possible assumptions
that may be made. To the best of our knowledge, these assumptions cover most of the TM implementations that are subject
to the validation step-complexity~\cite{HLM+03,norec,DSS06}.

It is easy to see that the lower bound of Theorem~\ref{th:iclb} is tight for both strict serializability and opacity.
We refer to the TM implementation in \cite{KR11-TR} or the popular \emph{DSTM}~\cite{HLM+03} that serves
as a matching upper bound. However, the quadratic step-complexity lower bound for opacity does not hold
under the assumption of weaker correctness conditions like strict serializability, 
\emph{virtual-world consistency}~\cite{damien-vw} and \emph{TMS1}~\cite{TMS}.

Finally, we conjecture that the lower bound of Theorem~\ref{th:mutex-tm-rmr} is tight. Proving this remains an interesting open
question.
%
